The pionic Drell-Yan process: a brief survey

The Drell-Yan process is an invaluable tool for probing the structure of hadrons, and the pion-induced Drell-Yan process is unique in its sensitivity to several subtleties of the partonic structure. This is a brief review of the pionic Drell-Yan process with particular emphasis on the dilepton angular distributions and nuclear modification of the parton distributions (the EMC effect).

==> epsfsafe.tex <==
%   EPSF.TEX macro file (modified for EPSF images with TIFF preview)
%
%   Written by Tomas Rokicki of Radical Eye Software, 29 Mar 1989.
%   Revised by Don Knuth, 3 Jan 1990.
%   Revised by Tomas Rokicki to accept bounding boxes with no
%	space after the colon, 18 Jul 1990.
%-%   Modified to deal with %%BoundingBox: (at end) as well as TIFF 
%-%	preview in EPSF format files, 1993 Jan 23 (see %-% comments).
%
%   TeX macros to include an Encapsulated PostScript graphic.
%   Works by finding the bounding box comment,
%   calculating the correct scale values, and inserting a vbox
%   of the appropriate size at the current position in the TeX document.
%
%   To use with the center environment of LaTeX, preface the \epsffile
%   call with a \leavevmode.  (LaTeX should probably supply this itself
%   for the center environment.)
%
%   To use, simply say
%   \input epsfsafe	  % somewhere early on in your TeX file
%   \epsfbox{filename.ps} % where you want to insert a vbox for a figure
%
%   Alternatively, you can type
%
%   \epsfbox[0 0 30 50]{filename.ps} % to supply your own BB
%
%   which will not read in the file, and will instead use the bounding
%   box you specify.
%
%   The effect will be to typeset the figure as a TeX box, at the
%   point of your \epsfbox command. By default, the graphic will have its
%   `natural' width (namely the width of its bounding box, as described
%   in filename.ps). The TeX box will have depth zero.
%
%   You can enlarge or reduce the figure by saying
%     \epsfxsize=<dimen> \epsfbox{filename.ps}
%   (or
%     \epsfysize=<dimen> \epsfbox{filename.ps})
%   instead. Then the width of the TeX box will be \epsfxsize and its
%   height will be scaled proportionately (or the height will be
%   \epsfysize and its width will be scaled proportiontally).  The
%   width (and height) is restored to zero after each use.
%
%   A more general facility for sizing is available by defining the
%   \epsfsize macro.  Normally you can redefine this macro
%   to do almost anything.  The first parameter is the natural x size of
%   the PostScript graphic, the second parameter is the natural y size
%   of the PostScript graphic.  It must return the xsize to use, or 0 if
%   natural scaling is to be used.  Common uses include:
%
%      \epsfxsize  % just leave the old value alone
%      0pt	   % use the natural sizes
%      #1	   % use the natural sizes
%      \hsize	   % scale to full width
%      0.5#1	   % scale to 50% of natural size
%      \ifnum#1>\hsize\hsize\else#1\fi	% smaller of natural, hsize
%
%   If you want TeX to report the size of the figure (as a message
%   on your terminal when it processes each figure), say `\epsfverbosetrue'.
%
\chardef\quoteleftcode=\catcode96	% remember catcode of `
\catcode96=12				% make sure ` is "ordinary"

\newread\epsffilein    % file to \read
\newif\ifepsffileok    % continue looking for the bounding box?
\newif\ifepsfbbfound   % success?
\newif\ifepsfverbose   % report what you're making?
\newdimen\epsfxsize    % horizontal size after scaling
\newdimen\epsfysize    % vertical size after scaling
\newdimen\epsftsize    % horizontal size before scaling
\newdimen\epsfrsize    % vertical size before scaling
\newdimen\epsftmp      % register for arithmetic manipulation
\newdimen\pspoints     % conversion factor
%
\pspoints=1bp	       % Adobe points are `big'
\epsfxsize=0pt	       % Default value, means `use natural size'
\epsfysize=0pt	       % ditto
%
\def\epsfbox#1{\global\def\epsfllx{72}\global\def\epsflly{72}%
   \global\def\epsfurx{540}\global\def\epsfury{720}%
   \def\lbracket{[}\def\testit{#1}\ifx\testit\lbracket
   \let\next=\epsfgetlitbb\else\let\next=\epsfnormal\fi\next{#1}}%
%
\def\epsfgetlitbb#1#2 #3 #4 #5]#6{\epsfgrab #2 #3 #4 #5 .\\%
   \epsfsetgraph{#6}}%
%
\def\epsfnormal#1{\epsfgetbb{#1}\epsfsetgraph{#1}}%
%
\def\epsfgetbb#1{%
%
%   The first thing we need to do is to open the
%   PostScript file, if possible.
%
\openin\epsffilein=#1
\ifeof\epsffilein\errmessage{I couldn't open #1, will ignore it}\else
%
%   Okay, we got it. Now we'll scan lines until we find one that doesn't
%   start with %. We're looking for the bounding box comment.
%
   {\epsffileoktrue \chardef\other=12
    \def\do##1{\catcode`##1=\other}\dospecials \catcode`\ =10
%-% Neuter some more nasty characters
    \catcode`\^^L=9 \catcode`\^^?=9
    \loop
       \read\epsffilein to \epsffileline
       \ifeof\epsffilein\epsffileokfalse\else
%
%   We check to see if the first character is a % sign;
%   if not, we stop reading (unless the line was entirely blank);
%   if so, we look further and stop only if the line begins with
%   `%%BoundingBox:'.
%
	  \expandafter\epsfaux\epsffileline:. \\%
       \fi
   \ifepsffileok\repeat
   \ifepsfbbfound\else
    \ifepsfverbose\message{No bounding box comment in #1; using defaults}\fi\fi
   }\closein\epsffilein\fi}%
%
%   Now we have to calculate the scale and offset values to use.
%   First we compute the natural sizes.
%
\def\epsfclipstring{}% do we clip or not?  If so,
\def\epsfclipon{\def\epsfclipstring{ clip}}%
\def\epsfclipoff{\def\epsfclipstring{}}%
%
\def\epsfsetgraph#1{%
   \epsfrsize=\epsfury\pspoints
   \advance\epsfrsize by-\epsflly\pspoints
   \epsftsize=\epsfurx\pspoints
   \advance\epsftsize by-\epsfllx\pspoints
%
%   If `epsfxsize' is 0, we default to the natural size of the picture.
%   Otherwise we scale the graph to be \epsfxsize wide.
%
   \epsfxsize\epsfsize\epsftsize\epsfrsize
   \ifnum\epsfxsize=0 \ifnum\epsfysize=0
      \epsfxsize=\epsftsize \epsfysize=\epsfrsize
      \epsfrsize=0pt
%
%   We have a sticky problem here:  TeX doesn't do floating point arithmetic!
%   Our goal is to compute y = rx/t. The following loop does this reasonably
%   fast, with an error of at most about 16 sp (about 1/4000 pt).
%
     \else\epsftmp=\epsftsize \divide\epsftmp\epsfrsize
       \epsfxsize=\epsfysize \multiply\epsfxsize\epsftmp
       \multiply\epsftmp\epsfrsize \advance\epsftsize-\epsftmp
       \epsftmp=\epsfysize
       \loop \advance\epsftsize\epsftsize \divide\epsftmp 2
       \ifnum\epsftmp>0
          \ifnum\epsftsize<\epsfrsize\else
	     \advance\epsftsize-\epsfrsize \advance\epsfxsize\epsftmp \fi
       \repeat
       \epsfrsize=0pt
     \fi
   \else \ifnum\epsfysize=0
     \epsftmp=\epsfrsize \divide\epsftmp\epsftsize
     \epsfysize=\epsfxsize \multiply\epsfysize\epsftmp
     \multiply\epsftmp\epsftsize \advance\epsfrsize-\epsftmp
     \epsftmp=\epsfxsize
     \loop \advance\epsfrsize\epsfrsize \divide\epsftmp 2
     \ifnum\epsftmp>0
	\ifnum\epsfrsize<\epsftsize\else
	   \advance\epsfrsize-\epsftsize \advance\epsfysize\epsftmp \fi
     \repeat
     \epsfrsize=0pt
    \else
     \epsfrsize=\epsfysize
    \fi
   \fi
%
%  Finally, we make the vbox and stick in a \special that dvips can parse.
%
   \ifepsfverbose\message{#1: width=\the\epsfxsize, height=\the\epsfysize}\fi
   \epsftmp=10\epsfxsize \divide\epsftmp\pspoints
   \vbox to\epsfysize{\vfil\hbox to\epsfxsize{%
      \ifnum\epsfrsize=0\relax
        \special{PSfile=#1 llx=\epsfllx\space lly=\epsflly\space
            urx=\epsfurx\space ury=\epsfury\space rwi=\number\epsftmp
            \epsfclipstring}%
      \else
        \epsfrsize=10\epsfysize \divide\epsfrsize\pspoints
        \special{PSfile=#1 llx=\epsfllx\space lly=\epsflly\space
            urx=\epsfurx\space ury=\epsfury\space rwi=\number\epsftmp\space
            rhi=\number\epsfrsize \epsfclipstring}%
      \fi
      \hfil}}%
\global\epsfxsize=0pt\global\epsfysize=0pt}%
%
%   We still need to define the tricky \epsfaux macro. This requires
%   a couple of magic constants for comparison purposes.
%
{\catcode`\%=12 \global\let\epsfpercent=%\global\def\epsfbblit{%BoundingBox}}%
%
%   So we're ready to check for `%BoundingBox:' and to grab the
%   values if they are found.
%
\long\def\epsfaux#1#2:#3\\{\ifx#1\epsfpercent
   \def\testit{#2}\ifx\testit\epsfbblit
      \epsfgrab #3 . . . \\%
      \epsffileokfalse
      \global\epsfbbfoundtrue
%-% Don't stop if line does not start with %.  May be (at end) or binary stuff
%  \fi\else\ifx#1\par\else\epsffileokfalse\fi\fi}%
   \fi\else\ifx#1\par\else\fi\fi}%
%
%   Here we grab the values and stuff them in the appropriate definitions.
%
\def\epsfempty{}%
\def\epsfgrab #1 #2 #3 #4 #5\\{%
\global\def\epsfllx{#1}\ifx\epsfllx\epsfempty
      \epsfgrab #2 #3 #4 #5 .\\\else
   \global\def\epsflly{#2}%
   \global\def\epsfurx{#3}\global\def\epsfury{#4}\fi}%
%
%   We default the epsfsize macro.
%
\def\epsfsize#1#2{\epsfxsize}
%
%   Finally, another definition for compatibility with older macros.
%
\let\epsffile=\epsfbox

\catcode`\`=\quoteleftcode		% restore previous catcode

==> referencejcp.tex <==
\bibitem{drell70} S.D. Drell and T.M. Yan, Phys. Rev. Lett. {\bf 25}, 316
   (1970); Ann. Phys. (NY) {\bf 66}, 578 (1971).
\bibitem {conrad98} J.M. Conrad, M.H. Shaevitz and T. Bolton,
Rev. Mod. Phys. {\bf 70} (1998) 1341.
\bibitem {gott} K. Gottfried, Phys. Rev. Lett. {\bf 18} (1967) 1174.
\bibitem {nmc91} P. Amaudruz {\it et al.}, Phys. Rev. Lett. {\bf 66} (1991)
2712.
\bibitem{e866} E.H. Hawker {\it et al.},  Phys. Rev.  Lett. {\bf 80} (1998)
3715.
\bibitem{peng} J.C. Peng {\it et al.}, Phys. Rev. {\bf D58} (1998) 092004.
\bibitem{towell} R.S. Towell {\it et al.}, Phys. Rev. {\bf D64} (2001) 052002.
\bibitem{kumano98} S. Kumano, Phys. Rep. {\bf 303} (1998) 183.
\bibitem{garvey02} G.T. Garvey and J.C. Peng, Prog. Part. Nucl. Phys. 
{\bf 47} (2001) 203.
\bibitem {thomas83} A. W. Thomas, Phys. Lett. {\bf B126} (1983) 97.
\bibitem {sullivan} J. D. Sullivan, Phys. Rev. {\bf D5} (1972) 1732.
\bibitem{e906} E906 Collaboration, D.F. Geesaman {\it et al.}, Fermi
National Accelerator Laboratory Proposal E906, 1999.
\bibitem{peng00} J.C. Peng, S. Sawada {\it et al.}, hep-ph/0007341.
\bibitem{ma1} B.Q. Ma, Phys. Lett. {\bf B274} (1992) 111.
\bibitem{boros} C. Boros, J.T. Londergan and A.W. Thomas, Phys. Rev. Lett.
{\bf 81} (1998) 4075.
\bibitem{peng1} J.C. Peng and D.M. Jansen, Phys. Lett. {\bf B354} (1995) 460.
\bibitem{yang09} R. Yang, J.C. Peng and M. Grosse-Perdekamp, Phys. Lett. 
{\bf B680} (2009) 231.
\bibitem{stirling93} W.J. Stirling and M.R. Whalley, J. Phys. {\bf G19},
       D1 (1993).
\bibitem{pat99} P.L. McGaughey, J.M. Moss, and J.C. Peng, Annu. Rev.
      Nucl. Part. Sci. {\bf 49}, 217 (1999).
\bibitem{kenyon82} I.R. Kenyon, Rep. Prog. Phys. {\bf 45}, 1261 (1982);
K. Freudenreich, Int. J. Mod. Phys. {\bf A5}, 3643 (1990).
\bibitem{lam78} C.S. Lam and W.K. Tung, Phys. Rev. {\bf D18}, 2447 (1978).
\bibitem{chiappetta86} P. Chiappetta and M. LeBellac, Z. Phys. {\bf C32}, 
521 (1986).
\bibitem{cleymans81} J. Cleymans and M. Kuroda, Phys. Lett. {\bf B105},
68 (1981).
\bibitem{callan69} C.G. Callan and D. J. Gross, Phys. Rev. Lett. {\bf 22},
    156 (1969).
\bibitem{lam80} C.S. Lam and W.K. Tung, Phys. Rev. {\bf D21}, 2712 (1980).
\bibitem{falciano86} NA10 Collaboration, S. Falciano {\em et al.}, Z. Phys.
    {\bf C31}, 513 (1986); M. Guanziroli {\em et al.},
    Z. Phys. {\bf C37}, 545 (1988).
\bibitem{conway89} E615 Collaboration, J.S. Conway {\em et al.}, Phys.
    Rev. {\bf D39}, 92 (1989); J.G. Heinrich {\em et al.}, Phys. Rev.
        {\bf D44}, 1909 (1991).
\bibitem{brandenburg93} A. Brandenburg, O. Nachtmann, and E. Mirkes, Z. Phys.
    {\bf C60}, 697 (1993).
\bibitem{boer05} D. Boer, A. Brandenburg, O. Nachtmann, and A. Utermann,
    Eur. Phys. J. {\bf C40}, 55 (2005).
\bibitem{brandenburg94} A. Brandenburg, S.J. Brodsky, V.V. Khoze,
and D. M\"{u}ller, Phys. Rev. Lett.
    {\bf 73}, 939 (1994).
\bibitem{eskola94} K.J. Eskola, P. Hoyer, M. V\"{a}ntinnen, and R.
Vogt, Phys. Lett. {\bf B333}, 526
    (1994).
\bibitem{berger79} E.L. Berger and S.J. Brodsky, Phys. Rev. Lett. {\bf 42},
    940 (1979).
\bibitem{boer99} D. Boer, Phys. Rev. {\bf D60}, 014012 (1999).
\bibitem{boer98} D. Boer and P.J. Mulders, Phys. Rev. {\bf D57},
    5780 (1998).
\bibitem{brodsky02} S.J. Brodsky, D.S. Hwang, and I. Schmidt, Phys.
        Lett. {\bf B530}, 99 (2002).
\bibitem{collins93} J.C. Collins, Nucl. Phys. {\bf B396}, 161 (1993).
\bibitem{gamberg03} L.P. Gamberg, G.R. Goldstein, and K.A. Oganessyan,
    Phys. Rev. {\bf D67}, 071504(R) (2003).
\bibitem{boer03} D. Boer, S.J. Brodsky, and D.S. Hwang, Phys. Rev. {\bf D67},
    054003 (2003).
\bibitem{bacchetta04} A. Bacchetta, A. Sch\"{a}fer, and J.-J. Yang, Phys.
    Lett. {\bf B578}, 109 (2004).
\bibitem{lu05} Z. Lu and B.-Q. Ma, Phys. Lett. {\bf B615}, 200 (2005).

\bibitem{brodsky80} S.J. Brodsky, P. Hoyer, C. Peterson, and N. Sakai,
Phys. Lett. B {\bf 93}, 451 (1980); S.J. Brodsky, C. Peterson, and
N. Sakai, Phys. Rev. D {\bf 23}, 2745 (1981).

\bibitem{pumplin06} J. Pumplin, Phys. Rev. D {\bf 73}, 114015 (2006);
J. Pumplin, H. L. Lai, and W. K. Tung, Phys.  Rev. D {\bf 75}, 054029
(2007).

%\bibitem{pumplin07} J. Pumplin, H. L. Lai, and W. K. Tung, Phys.
%Rev. D {\bf 75}, 054029 (2007).

\bibitem{e866} E. A. Hawker {\it et al.} (E866/NuSea
Collaboration), Phys. Rev. Lett. {\bf 80}, 3715 (1998);
J. C. Peng {\it et al.}, Phys. Rev. D {\bf 58}, 092004 (1998);
R.S. Towell {\it et al.}, Phys. Rev. D {\bf 64}, 052002 (2001).

\bibitem{hermes} A. Airapetian {\it et al.} (HERMES Collaboration),
Phys. Lett. B {\bf 666}, 446 (2008).

\bibitem{donoghue77} J. F. Donoghue and E. Golowich, Phys.
Rev. D {\bf 15}, 3421 (1977).


